Scaling VANET Security Through Cooperative Message Verification

VANET security introduces significant processing overhead for resource-constrained On-Board Units (OBUs). Here, we propose a novel scheme that allows secure Vehicular Communication (VC) systems to scale well beyond network densities for which existing optimization approaches could be workable, without compromising security (and privacy).

==> sections/model.tex <==
\section{System \& Adversary Model}

\subsection{System Model}

Vehicles (we refer to nodes in the rest of the paper) are able to communicate with road-side infrastructures (\ac{V2I} communication) and other vehicles (\ac{V2V} communication) over IEEE 802.11p wireless network. Vehicles broadcasts \acp{CAM} and \acp{DENM}~\cite{cam,denm} to inform the presence of themselves and alert hazardous events to their neighbors respectively. The frequency of \ac{CAM} messages ranges from $1$ $Hz$ to $10$ $Hz$ based on context of the vehicle, while we assume a 10 $Hz$ frequency in this paper as a demanding case.

We assume single-hop communication of broadcasted messages: the receivers of broadcasted messages will not relay/rebroadcast the messages. In addition, we assume each message is broadcasted by the message generator only once: there is no ACK of received packets or retransmission of any lost packets.

Legit nodes in the systems are equipped with short-term credentials (pseudonyms) that obtained from \ac{VPKI}~\cite{khodaei2014towards}. The integrity and authentication of messages are ensured by singing under the pseudonyms. 

\subsection{Adversary Model}

Consider the openness of wireless network, we assume a node (or an IEEE 802.11p enabled device) is able to broadcast/unicast any message in the network. A node that holds the private keys of valid credentials is able to use them as it wishes. A node is able to listen to all open communication in the system. We are concerned with adversaries that generate bogus message and mislead their neighbors on the validity of the bogus messages, resulting in the acceptance of such messages through our scheme.

==> sections/problem.tex <==
\section{Problem Statement}

Vehicular communication introduce frequent \ac{V2I} and \ac{V2V} communication. Among others, we are interested in \ac{CAM} messages which ensures geographical awareness of each other. A node broadcast \ac{CAM} messages in the network which include status information, such as speed, location and direction. These messages are secured with short-lived credentials, which provide messages authentication and integrity while privacy is preserved. Generation and verification of such messages incur extra resource consumption to the node. The need of frequent expensive operations and the fact that each node has limited resource, implies that such messages can be handled only at limited rate.  This means if a node is saturated with excessive amount of messages; the waiting time of each message to get verified would get longer over time, thus the freshness of messages cannot be preserved.

In this paper, we are concerned with resource and time consumption of nodes on verifying signed messages. We seek to reduce significantly the overhead of message verification while incur reasonable overhead on communication and message generation. In addition, we want our scheme to be resilient to malicious nodes in the system: the system should be able to identify and reveal the malicious nodes cooperatively.

While we increase efficiency on message verification, we do not compromise any security and privacy requirements in \ac{VC}, notably non-repudiation and unlinkability/pseudonymity.


==> sections/related.tex <==
\section{Related Works???}

\begin{comment}
	\item Cooperative Message Authentication - similar idea, but with customized cryptography, i.e., not standard compliant \& not consider performance \cite{lin2013achieving}
	\item Batch verification
	\item Certificate omission
	\item Group based protocol
	\item Eviction based on bloom filter
\end{comment}
